A bit better: Variants of duality in geometric algebras with degenerate metrics

Multiplication by the pseudoscalar $\mathbf{I}$ has been traditionally used in geometric algebra to perform non-metric operations such as calculating coordinates and the regressive product. In algebras with degenerate metrics, such as euclidean PGA $P(\mathbb{R}^*_{3,0,1})$, this approach breaks down, leading to a search for non-metric forms of duality. The article compares the dual coordinate map $J: G \rightarrow G^*$, a double algebra duality, and Hodge duality $H: G \rightarrow G $, a single algebra duality for this purpose. While the two maps are computationally identical, only $J$ is coordinate-free and provides direct support for geometric duality, whereby every geometric primitive appears twice, once as a point-based and once as a plane-based form, an essential feature not only of projective geometry but also of euclidean kinematics and dynamics. Our analysis concludes with a proposed duality-neutral software implementation, requiring a single bit field per multi-vector.

==> GunnMac.tex <==

\usepackage{xspace}
\usepackage{helvet}
\usepackage{courier}
%
\usepackage{fancyhdr}
\usepackage{type1cm}         
\usepackage{subeqnarray}
%\usepackage{makeidx}         % allows index generation
\usepackage{graphicx}        % standard LaTeX graphics tool
                             % when including figure files
%\usepackage{multicol}        % used for the two-column index
%\usepackage[bottom]{footmisc}% places footnotes at page bottom
%\usepackage{amscd}	% commutative diagrams
\usepackage{enumerate}
% following disturbs capital greek letters in math mode!
%\usepackage{mathptmx}       % selects Times Roman as basic font
%\usepackage{wsuipa}   % to get a widetilde symbol
\usepackage{amsmath, latexsym}
%\usepackage{cgg}
\usepackage{array}
\usepackage{tabularx}
\usepackage{url}
\usepackage{relsize}
\usepackage{ifthen}
\usepackage{xcolor}
\usepackage[newitem,newenum]{paralist}
\def\isExcerpt{false} 
\def\isBeamer{false}

\newcommand{\mychapterskip}{\ifthenelse{\equal{\isMPK}{true}}
{\vspace{-.8in}}{}}

\newcommand{\correction}{} %{\marginpar{Corrected since 22.12.10}}
\newcommand{\blackfbox}[1]{\setlength{\fboxsep{0pt}\fbox{{#1}}}}
\newcommand{\fullversion}{\cite{gunnFull2010}\xspace}
\newcommand{\fullversioncolor}{\color{black!50!blue}}
\newcommand{\versions}[2]{\ifthenelse{\equal{\isfullversion}{true}}{{\fullversioncolor#1}}{#2}}
% see the list of further useful packages
% in the Reference Guide

%\makeindex             % used for the subject index
                       % please use the style svind.ist with
                       % your makeindex program
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\quot}[1]{``#1''}
\newcommand{\INP}[2]{\langle #1, #2 \rangle}
\newcommand{\R}[1]{\ensuremath{\mathbb{R}^{#1}\xspace}}
\newcommand{\Euc}[1]{\ensuremath{\mathbf{E}^{#1}\xspace}}
\newcommand{\Eucg}[1]{\ensuremath{E(#1)\xspace}}
\newcommand{\Eucgd}[1]{\ensuremath{E^+(#1)\xspace}}
\newcommand{\DEuc}[1]{\ensuremath{\mathbf{E}^{#1*}\xspace}}
\newcommand{\DEucg}[1]{\ensuremath{{E}(#1)^*\xspace}}
\newcommand{\RD}[1]{\ensuremath{(\mathbb{R}^{#1})^{*}\xspace}}
\newcommand\proj[1]{\ensuremath{\mathbf{P}(#1)}\xspace}
\newcommand\RP[1]{\ensuremath{\mathbb{R}{P^{#1}}\xspace}}
\newcommand\RPD[1]{\ensuremath{(\mathbb{R}{P^{#1}})^{*}\xspace}}
\newcommand{\Sph}[1]{\ensuremath{\mathbf{S}^{#1}\xspace}}
\newcommand{\Ell}[1]{\ensuremath{\mathbf{Ell}^{#1}\xspace}}
\newcommand{\Hyp}[1]{\ensuremath{\mathbf{H}^{#1}\xspace}}
\newcommand{\DHyp}[1]{\ensuremath{\mathbf{H}^{#1 *}\xspace}}
\newcommand{\e}[1]{\vec{e}_{#1}}
\newcommand{\EE}[1]{\vec{E}_{#1}}
\newcommand{\one}{\vec{1}}
\newcommand{\eye}{\vec{I}}
\newcommand{\inert}{\mathbf{A}}
\newcommand{\stripeye}[1]{\ensuremath{\mathbf{S}(#1)}}
\newcommand{\noneuc}{non-euclidean\xspace}
\newcommand{\Noneuc}{Non-euclidean\xspace}
\newcommand{\MN}{metric-neutral\xspace}
\newcommand{\Mn}{Metric-neutral}
\newcommand{\CR}{}	% cross-ratio: omit any name
%\newcolumntype{Y}{>{\center}X}
\newcolumntype{Y}{X}
\newcommand{\ctrt}{\bot}
\newcommand{\inpro}{\cdot}
\newcommand{\beam}{spear}
\newcommand{\bivo}[1]{{\vec{#1}}}
\newcommand{\pip}{\bivo{\Xi}}
\newcommand{\piper}{\pip^\perp}
\newcommand{\psip}{\bivo{\Psi}}
\newcommand{\omp}{\bivo{\Lambda}}
\newcommand{\pvelo}{\bivo{\Gamma}}
\newcommand{\velo}{\bivo{\Omega}}
\newcommand{\momo}{\bivo{\Pi}}
\newcommand{\foro}{\bivo{\Delta}}
\newcommand{\sigo}{\bivo{\Sigma}}
\newcommand{\fio}{\bivo{\Phi}}
\newcommand{\thio}{\bivo{\Theta}}
\newcommand{\hard}{${}^*$}
\newcommand{\grade}[2]{\langle #1 \rangle_{#2}}
\newcommand{\grass}[1]{\bigwedge{\mathbb{R}^{#1}}}
\newcommand{\grassgr}[2]{\bigwedge^{#2}{\mathbb{R}^{#1}}}
\newcommand{\dgrass}[1]{\bigwedge{\mathbb{R}^{#1*}}}
\newcommand{\pgrass}[1]{\proj{\bigwedge{\mathbb{R}^{#1}}}}
\newcommand{\pdgrass}[1]{\proj{\bigwedge({\mathbb{R}^{#1})^*}}}
\newcommand{\pgrassgr}[2]{\proj{\bigwedge^{#2}{\mathbb{R}^{#1}}}}
\newcommand{\pdgrassgr}[2]{\proj{\bigwedge^{#2}({\mathbb{R}^{#1})^*}}}
\newcommand{\pgrassv}{\proj{\bigwedge{\VS}}}
\newcommand{\pdgrassv}{\proj{\bigwedge{\VS^{*}}}}
\newcommand{\pgrassgrv}[1]{\ensuremath{\proj{\bigwedge^{#1}{\VS}}}}
\newcommand{\pdgrassgrv}[1]{\ensuremath{\proj{\bigwedge^{#1}\VS^{*}}}}
\newcommand{\claltwo}[2]{\mathbb{R}_{#1,#2}\xspace}
\newcommand{\clal}[3]{\mathbb{R}_{#1,#2,#3}\xspace}
\newcommand{\dclal}[3]{\mathbb{R}^*_{#1,#2,#3}\xspace}
\newcommand{\pclaltwo}[2]{\proj{\claltwo{#1,#2}}}
\newcommand{\pclal}[3]{\proj{\mathbb{R}_{#1,#2,#3}}\xspace}
\newcommand{\pdclal}[3]{\proj{\mathbb{R}^*_{#1,#2,#3}}\xspace}
\newcommand{\dclplus}[3]{{\mathbb{R}^{*+}_{#1,#2,#3}}\xspace}
\newcommand{\pdclplus}[3]{\proj{\mathbb{R}^{*+}_{#1,#2,#3}}\xspace}
\newcommand{\pclplus}[3]{\proj{\mathbb{R}^{+}_{#1,#2,#3}}\xspace}
\newcommand{\spin}[3]{\mathbf{Spin}({#1,#2,#3})}
\newcommand{\spineps}{\mathbf{Spin}_{\kappa}}
\newcommand{\espin}[1]{\mathbf{Spin}^{#1}_{+\kappa}}
\newcommand{\espinx}[2]{\mathbf{Spin}^{#1}_{+#2}}
\newcommand{\epin}[1]{\mathbf{Pin}^{#1}_{+\kappa}}
\newcommand{\efspin}[1]{\mathbf{Spin}^{#1}_{\kappa}}
\newcommand{\ecl}[1]{\ensuremath{Cl^{#1}_{\kappa}}}
\newcommand{\eclx}[2]{\ensuremath{Cl^{#1}_{#2}}}
\newcommand{\epcl}[1]{\ensuremath{Cl^{#1 +}_{\kappa}}}
\newcommand{\epclx}[2]{\ensuremath{Cl^{#1 +}_{#2}}}
\newcommand{\escl}[1]{\ensuremath{Cl^{#1 \dag}_{\kappa}}}
\newcommand{\esclx}[2]{\ensuremath{Cl^{#1 \dag}_{#2}}}
\newcommand{\liealg}{\ensuremath{\mathfrak{g}}}
\newcommand{\liegrp}{\ensuremath{\mathbf{G}}}
\newcommand{\kurv}{\ensuremath{\kappa}}
\newcommand{\de}{dual euclidean\xspace}
\newcommand{\De}{Dual euclidean\xspace}
\newcommand{\motion}{isometric motion\xspace}
\newcommand{\stnm}{Study number\xspace}
\newcommand{\stnms}{Study numbers\xspace}
\newcommand{\rotorisom}[1]{\ensuremath{\underline{#1}}\xspace}
\newcommand{\plperp}[1]{\ensuremath{#1^{\vdash}}}
\newcommand{\metpol}{\ensuremath{\eye}\xspace}
\newcommand{\metpolf}[1]{\ensuremath{\eye(#1)}\xspace}
\newcommand{\exerc}{\subsubsection{Examples}}
\newcommand{\linespace}{\ensuremath{\mathcal{L}}\xspace}%\mathbf{M}^4_2} \xspace} %\mathbf{L}^{3,3}}\xspace}
\newcommand{\complexspace}{\ensuremath{\mathfrak{B}}\xspace}
\newcommand{\adjoint}{adjoint\xspace}
\newcommand{\VS}{\ensuremath{\mathsf{V}}}
\newcommand{\VSD}{\ensuremath{\mathsf{V}^{*}}}
\newcommand{\PVS}{\proj{\VS}}
\newcommand{\PVSD}{\proj{\VSD}}
\newcommand{\vtx}[1]{\ensuremath{\mathcal{V}_{#1}}}
\newcommand{\Det}{\ensuremath{\bigtriangleup}}
\newcommand{\W}{\pgrassv}
\newcommand{\WD}{\pdgrassv}
\newcommand{\adj}[1]{{#1}^{*}}
\newcommand{\myexercise}{\hspace{-.31in}\textbf{Exercise:~~\xspace}}
\newcommand{\myexercises}{\hspace{-.31in}\textbf{Exercises:~~\xspace}}
\newcommand{\myboldhead}[1]{\vspace{0in}\hspace{0in}\textbf{#1.}}
\newcommand{\myparagraph}[1]{\hspace{-.0in}\textbf{#1.}}%{\paragraph{#1}} %
\newcommand{\mysubsubsection}[1]{\subsubsection{#1}}%{\hspace{-.0in}\textbf{#1.}}%
\newcommand{\mymarginpar}[1]{\marginpar{#1}} %{}%
\newcommand{\remarko}{\remark\xspace} %\mysubsubsection{Remark}\xspace}
\newcommand{\lremarko}[1]{\remarko\hspace{-.0in}\textbf{#1}} 
\newcommand{\orientref}{\Sec{sec:orientation}}
\newcommand{\nebenachse}{secondary axis\xspace}
\newcommand{\foreward}{the Foreward}
\newcommand{\myintro}{Preface}
\newcommand{\app}[1]{\Sec{sec:J}}
\newcommand{\red}[1]{{\color{red} #1}}
\newcommand{\blue}[1]{{\color{blue} #1}}
\definecolor{mypurple}{rgb}{1,0,1}
\newcommand{\purple}[1]{{\color{mypurple} #1}}
\definecolor{mygreen}{rgb}{0, .5, 0}
\newcommand{\green}[1]{{\color{mygreen} #1}}

\newcommand{\Ex}[2]{Ex.~\ref{#1}-\ref{#2}}
\newcommand{\Def}[1]{Def.~\ref{#1}}
\newcommand{\Eq}[1]{(\ref{#1})}
\newcommand{\Fig}[1]{Fig.~\ref{#1}}
\newcommand{\Tab}[1]{Table~\ref{#1}}
\newcommand{\Sec}[1]{Sect.~\ref{#1}}
\newcommand{\Rem}[1]{Remark~\ref{#1}}
\newcommand{\Cor}[1]{Corollary~\ref{#1}}
\newcommand{\Thm}[1]{Thm.~\ref{#1}}
\ifthenelse{\equal{\isBeamer}{true}}
{
\renewcommand{\Theorem}[1]{Theorem~\ref{#1}}
\renewcommand{\Lemma}[1]{Lemma~\ref{#1}}}
{
\newcommand{\Theorem}[1]{Theorem~\ref{#1}}
\newcommand{\Lemma}[1]{Lemma~\ref{#1}}
}
\newcommand{\Ch}[1]{Chapter~\ref{#1}}
\newcommand{\mycorrection}[1]{}

% from GAMacros
\newcommand{\GA}{\ensuremath{{\cal G}}}
\newcommand{\Rs}[1]{\ensuremath{{\mathbb R}^{#1}}}
\newcommand{\Ra}[1]{\ensuremath{{\mathbb R}_{#1}}} 
\newcommand{\PRa}[1]{\ensuremath{\proj{{\mathbb R}_{#1}}} }
% alternative \newcommand{\Ra}[1] {\ensuremath{\GA(\Rs{#1})}} and the like
\newcommand{\Rag}[2]{\ensuremath{{{\mathbb R}_{#1}^{#2}}}}
\newcommand{\Rae}[1]{\ensuremath{{{\mathbb R}_{#1}^+}}}
\newcommand{\Rao}[1]{\ensuremath{{{\mathbb R}_{#1}^-}}}
\newcommand{\CGAs}{\ensuremath{{\mathbb R}^{4,1}}}
\newcommand{\CGAa}{\ensuremath{\proj{\mathbb{R}_{4,1}}}}
\newcommand{\CGAg}[1]{\ensuremath{{\mathbb R}_{4,1}^{#1}}}
\newcommand{\CGAe}{\ensuremath{{{\mathbb R}_{4,1}^+}}}
\newcommand{\CGAo}{\ensuremath{{{\mathbb R}_{4,1}^-}}}


